Congestion Control Mechanisms for Inter-Datacenter Networks

Applications running in geographically distributed setting are becoming prevalent. Large-scale online services often share or replicate their data into multiple data centers (DCs) in different geographic regions. Driven by the data communication need of these applications, inter-datacenter network (IDN) is getting increasingly important. However, we find congestion control for inter-datacenter networks quite challenging. Firstly, the inter-datacenter communication involves both data center networks (DCNs) and wide-area networks (WANs) connecting multiple data centers. Such a network environment presents quite heterogeneous characteristics (e.g., buffer depths, RTTs). Existing congestion control mechanisms consider either DCN or WAN congestion, while not simultaneously capturing the degree of congestion for both. Secondly, to reduce evolution cost and improve flexibility, large enterprises have been building and deploying their wide-area routers based on shallow-buffered switching chips. However, with legacy congestion control mechanisms (e.g., TCP Cubic), shallow buffer can easily get overwhelmed by large BDP (bandwidth-delay product) wide-area traffic, leading to high packet losses and degraded throughput. This thesis describes my research efforts on optimizing congestion control mechanisms for the inter-datacenter networks. First, we design GEMINI - a practical congestion control mechanism that simultaneously handles congestions both in DCN andWAN. Second, we present FlashPass - a proactive congestion control mechanism that achieves near zero loss without degrading throughput under the shallow-buffered WAN. Extensive evaluation shows their superior performance over existing congestion control mechanisms.

==> chapters/gemini/abstract.tex <==
Geographically distributed applications hosted on cloud are becoming prevalent.
They run on \textit{cross-datacenter network} that consists of multiple data
center networks (DCNs) connected by a wide area network (WAN). Such a cross-DC
network poses significant challenges in transport design because the DCN and
WAN segments have vastly distinct characteristics (\eg, buffer depths, RTTs). 

In this paper, we find that existing DCN or WAN transport reacting to ECN or 
delay alone do not (and cannot be extended to) work well for such an environment. 
The key reason is that neither of the signals, by itself only, can simultaneously capture
the location and degree of congestion, mainly due to the discrepancies between
DCN and WAN. Motivated by this, we present the design and implementation of \sys
that strategically integrates both ECN and delay signals for cross-DC congestion
control. To achieve low latency, \sys bounds the inter-DC latency with delay
signal and prevents the intra-DC packet loss with ECN. To maintain high
throughput, \sys modulates the window dynamics and maintains low buffer
occupancy utilizing both congestion  signals. \sys is implemented in Linux
kernel and evaluated by extensive testbed experiments. \revise{Results show that \sys
achieves up to 53\%, 31\%, 76\% and 2\% reduction of small flow average completion
times, and up to 34\%, 39\%, 9\% and 58\% reduction of large
flow average completion times compared to TCP Cubic, DCTCP, BBR and TCP Vegas.}
%Finally, \sys requires no customized hardware support and thus can be readily
%deployed in practice.

